Asymmetric Streaming Algorithms for Edit Distance and LCS

The edit distance (ED) and longest common subsequence (LCS) are two fundamental problems which quantify how similar two strings are to one another. In this paper, we consider these problems in the asymmetric streaming model introduced by Andoni et al. (FOCS'10) and Saks and Seshadhri (SODA'13). In this model we have random access to one string and streaming access the other string. Our main contribution is a constant factor approximation algorithm for ED with the memory of $\tilde O(n^{\delta})$ for any constant $\delta > 0$. In addition to this, we present an upper bound of $\tilde O_\epsilon(\sqrt{n})$ on the memory needed to approximate ED or LCS within a factor $1+\epsilon$. All our algorithms are deterministic and run in a single pass. For approximating ED within a constant factor, we discover yet another application of triangle inequality, this time in the context of streaming algorithms. Triangle inequality has been previously used to obtain subquadratic time approximation algorithms for ED. Our technique is novel and elegantly utilizes triangle inequality to save memory at the expense of an exponential increase in the runtime.

==> streamingintroduction.tex <==
@inproceedings{SW07,
  author    = {Xiaoming Sun and
               David P. Woodruff},
  title     = {The communication and streaming complexity of computing the longest
               common and increasing subsequences},
  booktitle = {Proceedings of the Eighteenth Annual {ACM-SIAM} Symposium on Discrete
               Algorithms, {SODA} 2007, New Orleans, Louisiana, USA, January 7-9,
               2007},
  pages     = {336--345},
  year      = {2007},
  crossref  = {DBLP:conf/soda/2007},
  url       = {http://dl.acm.org/citation.cfm?id=1283383.1283419},
  timestamp = {Fri, 07 Dec 2012 17:02:09 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/soda/SunW07},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{CGK16,
 author = {Chakraborty, Diptarka and Goldenberg, Elazar and Kouck\'{y}, Michal},
 title = {Streaming Algorithms for Embedding and Computing Edit Distance in the Low Distance Regime},
 booktitle = {Proceedings of the Forty-eighth Annual ACM Symposium on Theory of Computing},
 series = {STOC '16},
 year = {2016},
 isbn = {978-1-4503-4132-5},
 location = {Cambridge, MA, USA},
 pages = {712--725},
 numpages = {14},
 url = {http://doi.acm.org/10.1145/2897518.2897577},
 doi = {10.1145/2897518.2897577},
 acmid = {2897577},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Edit distance, Hamming distance, kernel, low distortion, randomized embedding, string},
}


@article{LMS98,
 author = {Landau, Gad M. and Myers, Eugene W. and Schmidt, Jeanette P.},
 title = {Incremental String Comparison},
 journal = {SIAM J. Comput.},
 issue_date = {April 1998},
 volume = {27},
 number = {2},
 month = apr,
 year = {1998},
 issn = {0097-5397},
 pages = {557--582},
 numpages = {26},
 url = {http://dx.doi.org/10.1137/S0097539794264810},
 doi = {10.1137/S0097539794264810},
 acmid = {279125},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
 keywords = {dynamic programming, edit-distance, string matching},
}


@article{RS20,
  author    = {Aviad Rubinstein and
               Zhao Song},
  title     = {Reducing approximate Longest Common Subsequence to approximate Edit
               Distance},
  journal   = {CoRR},
  volume    = {abs/1904.05451},
  year      = {2019},
  url       = {http://arxiv.org/abs/1904.05451},
  archivePrefix = {arXiv},
  eprint    = {1904.05451},
  timestamp = {Thu, 25 Apr 2019 13:55:01 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1904-05451},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{AlonMS96,
 author = {Alon, Noga and Matias, Yossi and Szegedy, Mario},
 title = {The Space Complexity of Approximating the Frequency Moments},
 booktitle = {Proceedings of the Twenty-eighth Annual ACM Symposium on Theory of Computing},
 series = {STOC '96},
 year = {1996},
 isbn = {0-89791-785-5},
 location = {Philadelphia, Pennsylvania, USA},
 pages = {20--29},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/237814.237823},
 doi = {10.1145/237814.237823},
 acmid = {237823},
 publisher = {ACM},
 address = {New York, NY, USA},
}




@inproceedings{Demaine-Lopez-Ortiz-Munro-2002,
 author = {Demaine, Erik D. and L\'{o}pez-Ortiz, Alejandro and Munro, J. Ian},
 title = {Frequency Estimation of Internet Packet Streams with Limited Space},
 booktitle = {Proceedings of the 10th Annual European Symposium on Algorithms},
 series = {ESA '02},
 year = {2002},
 isbn = {3-540-44180-8},
 pages = {348--360},
 numpages = {13},
 url = {http://dl.acm.org/citation.cfm?id=647912.740658},
 acmid = {740658},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
}

@inproceedings{CCHM15,
  author    = {Rajesh Hemant Chitnis and
               Graham Cormode and
               Mohammad Taghi Hajiaghayi and
               Morteza Monemizadeh},
  title     = {Parameterized Streaming: Maximal Matching and Vertex Cover},
  booktitle = {Proceedings of the Twenty-Sixth Annual {ACM-SIAM} Symposium on Discrete
               Algorithms, {SODA} 2015, San Diego, CA, USA, January 4-6, 2015},
  pages     = {1234--1251},
  year      = {2015},
  crossref  = {DBLP:conf/soda/2015},
  url       = {https://doi.org/10.1137/1.9781611973730.82},
  doi       = {10.1137/1.9781611973730.82},
  timestamp = {Fri, 02 Nov 2018 09:33:56 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/soda/ChitnisCHM15},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{FKMSZ05,
 author = {Feigenbaum, Joan and Kannan, Sampath and McGregor, Andrew and Suri, Siddharth and Zhang, Jian},
 title = {On Graph Problems in a Semi-streaming Model},
 journal = {Theor. Comput. Sci.},
 issue_date = {8 December 2005},
 volume = {348},
 number = {2},
 month = dec,
 year = {2005},
 issn = {0304-3975},
 pages = {207--216},
 numpages = {10},
 url = {http://dx.doi.org/10.1016/j.tcs.2005.09.013},
 doi = {10.1016/j.tcs.2005.09.013},
 acmid = {1132638},
 publisher = {Elsevier Science Publishers Ltd.},
 address = {Essex, UK},
 keywords = {articulation point, girth, graph, matching, spanner, streaming},
}

\begin{abstract}
The \textit{edit distance} (\textsf{ED}) and \textit{longest common
sub-sequence} (\textsf{LCS}) problems are fundamental computer
science problems which  quantify how similar two strings are to one
another. In this paper, We present a constant as well as
$1+\epsilon$ approximation streaming algorithm for computing ED and
LCS with sublinear space for a natural model in which one pattern
string is already stored in a read-only storage. This is especially
motivated for streams of large strings for which we try to compare
with a large pattern string in a read-only memory. Indeed our
results in this paper strictly generalizes previous results on
longest increasing  sub-sequence as well as distance to
monotonicity. \textbf{XXX we should add more motivation for the
mode} \textbf{XXX we should flash out our results here }
\end{abstract}


\thispagestyle{empty} \setcounter{page}{0}
\section{Introduction}\label{introduction}
We consider \textit{edit distance} (\textsf{ED}) and \textit{longest
common subsequence} (\textsf{LCS}) which are  classic similarity
problems between two strings  and have been studied widely in
combinatorial optimization as well as computer science. Edit
distance is defined on two  strings $x$ and $y$ and seeks the
smallest number of character insertions, character deletions, and
character substitutions to transform $x$ into $y$. While in edit
distance the goal is to make a transformation, longest common
subsequence asks for the largest string that appears as a
subsequence in both $x$ and $y$.

Edit distance and longest common subsequence have applications in
various contexts, such as computational biology, text processing,
compiler optimization, data analysis, image analysis, among others.
As a result, both these problems have been subject to a plethora of
studies since 1950 (e.g. see
\textit{e.g.}~\cite{bellman1957dynamic,boroujeni2018approximating,abboud2015tight,backurs2015edit,andoni2012approximating,andoni2010polylogarithmic,indyk2001algorithmic,
    %bar2004approximating,
    batu2006oblivious,crochemore2001fast,
    de1999extensive,hunt1977fast,masek1980faster,
    crochemore2003subquadratic,gusfield1997algorithms,landau1998incremental,
    bringman2018multivariate,
    %apostolico1990efficient, mathies1988fast,alves2002parallel, aggarwal1988notes, lu1994parallel, babu1997parallel, lu1990parallel,garcia2003coarse, alves2003bsp,
     alves2006coarse,bestpaper,
    saha17, saha16, saha15, %saha14,
    saha172, saha19, amitkumarted, rabaniedit,
     lcs-hardness2, lcs-hardness3, edlcsmr, woodrufflcs, woodruffdtw, andonied1, smootheded, andonied2, andonied3, lcrs-journal,
     dwt, charikar2018estimating, dtw2, mike1, aviad1, abboud-lcs-hardness2, spaaedulam, hajiaghayi2019approximating,bestpaper}).

Big (text) data are everywhere nowadays. Examples include the genome
sequences, the world-wide web data, and (text) data and messages
owned by companies such as Facebook, LinkedIn, and Twitter.
Traditional algorithms often cannot address complexity of big data
which demand highly resource efficient algorithms. A poplar model
for handling big data is the {\em streaming} model in which  the
input arrives in a sequence of stream while we have only sublinear
space in terms of the input to process the input stream. The idea of
streaming algorithms is about two decades old
(\cite{AlonMS96,Demaine-Lopez-Ortiz-Munro-2002}) and other variants
such as the semi-streaming model~\cite{FKMSZ05} and parameterized
streaming~\cite{CCHM15} have been introduced as well. However there
is not much positive results for streaming algorithms of
\textsf{ED}\ and \textsf{LCS} which are possibly far away. In this
paper we make the first substantial improvements on streaming
algorithms for these two problems. In particular, we consider a
natural model in which one string streams and the other one is
stored in a read-only memory and we have a sublinear space to
process the streaming string.  This is especially motivated for
streams of large strings for which we try to compare with a large
pattern string in a read-only memory. Indeed we show this model
already generalizes other problems such as longest increasing
subsequence and  distance to monotonicity among others. We design
streaming algorithms with sublinear space for this streaming model
of \textsf{ED}\ and \textsf{LCS}.

\textbf{XXX we should add more motivation for the mode} \textbf{XXX
we should flash out our results here }

\section{Related work}
Quadratic time solutions for  \textsf{ED}\ and \textsf{LCS}\ have
been known for many decades and indeed a truly subquadratic time
solution for either \textsf{ED} or \textsf{LCS} refutes {\em Strong
Exponential Time Hypothesis} \textsf{SETH} a widely believed
conjecture
(see~\cite{backurs2015edit,abboud2015tight,lcs-hardness3}). Thus
approximation algorithms have also been  studied widely for these
two problems. For edit distance, a series of
works~\cite{landau1998incremental},~\cite{bar2004approximating},~\cite{batu2006oblivious},
and~\cite{andoni2012approximating} improve the approximation factor
culminating in the seminal work of Andoni, Krauthgamer, and
Onak~\cite{andoni2010polylogarithmic} that finally obtains a
polylogarithmic approximation in near-linear time. More recent
 first a quantum solution~\cite{boroujeni2018approximating}, and later a follow-up algorithm~\cite{bestpaper} which removes the quantum
 step obtain a {\em truly} subquadratic algorithm with a constant factor
 approximation for the \textsf{ED}.
\textsf{LCS} has also received tremendous  attention in recent
years~\cite{hajiaghayi2019approximating,rubinstein2019reducing,saeedfocs19,abboud-lcs-hardness1,
abboud-lcs-hardness2, cglrr18}. Only trivial solutions were known
for \textsf{LCS} until very recently: a 2 approximate solution when
the alphabet is 0/1 and an $O(\sqrt{n})$ approximate solution for
general alphabets in linear time. Both these bounds are recently
improved by Hajiaghayi \textit{et
al.}~\cite{hajiaghayi2019approximating} and Rubinstein and
Song~\cite{rubinstein2019reducing} (see also a recent approximation
algorithms given by Rubinstein \textit{et al.}~\cite{saeedfocs19}).

Parameterized streaming algorithms for edit distance has been
considered when the edit distance between the pair of strings  is
{\em bounded} by a parameter $k$ which is much less than $n$. The
best off-line algorithm runs in time $O(n+k^2)$~\cite{LMS98} which
is known to be optimal under \textsf{SETH}. A parameterized
streaming algorithm  that makes one-pass over its input $x$ and $y$
with space $O(k)$ (which can be as large as the input size) and
running time $O(n+k^4)$~\cite{CGK16} (STOC'16) (which is further
improvement to $O(n+k^2)$ by the arxiv version of the previous
paper)  is presented recently as well. Sun and Woodruff \cite{SW07}
consider streaming complexity of related but simpler problems of the
longest common and increasing subsequences. In particular they
obtain a streaming algorithm with space $O(\sqrt{n})$ with a
constant factor approximation for the increasing subsequence
problem. Our solution for edit distance strictly generalizes their
results as well.

\textbf{XXX I do not remember the paper that improves Sun and
Woodruff above. we should flash out their results more and say how
we generalize them }

\section{Our results and techniques}

